Stochastic processes on preferential attachment models

In real life, networks are dynamic in nature; they grow over time and often exhibit power-law degree sequences. To model the evolving structure of the internet, Barab\'{a}si and Albert introduced a simple dynamic model with a power-law degree distribution. This model has since been generalised, leading to a broad class of affine preferential attachment models, where each new vertex connects to existing vertices with a probability proportional to the current degree of the vertex. While numerous studies have explored the global and local properties of these random graphs, their dynamic nature and the dependencies in edge-connection probabilities have posed significant analytical challenges. The first part of this thesis identifies the local limit of preferential attachment models in considerable generality. The second part focuses on stochastic processes on preferential attachment models, introducing an additional layer of randomness to the random graphs. Examples of such processes include bond and site percolation, random walks, the Ising and Potts models, and Gaussian processes on random graphs. In this thesis, we specifically examine percolation and the Ising model, exploring these processes using the local limit identified earlier.

==> Back_matter/Publications.tex <==
\chapter*{ 
\vspace*{\emptychapterdist}List of publications}
\vspace{10pt}

\begin{itemize}
	\item Cipriani, A., Dan, B., Hazra, R.S., \& Ray, R. (2021). \textit{Maximum of the Membrane Model on Regular Trees}. Journal of Statistical Physics, Volume: 190, 1-32, doi: 10.1007/s10955-022-03043-w.
	\item Garavaglia, A., Hazra, R.S., van der Hofstad, R., \& Ray, R. (2022). \textit{Universality of the local limit of preferential attachment models}. arXiv Preprint, doi: 10.48550/arXiv.2212.05551.
	\item Hazra, R.S., van der Hofstad, R., \& Ray, R. (2023). \textit{Percolation on preferential attachment models}. arXiv  Preprint, doi: 10.48550/arXiv.2312.14085.
	\item van der Hofstad, R., \& Ray, R. (2024). \textit{Ising model on preferential attachment models}. In preparation.
	\item Hazra, R.S., van der Hofstad, R., \& Ray, R. (2024). \textit{Tiny giant in sub-critical preferential attachment models}. In preparation.
\end{itemize}

==> Chap1_Intro/PA.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preferential attachment models}\label{chap:intro:sec:PA}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The Barab\'asi-Albert model of \cite{ABrB,albert1999} is {one of the most popular random graph model for dynamic real-life networks} due to the fact that, through a simple dynamic, its properties resemble real-world networks. This model has been generalized in many different ways, creating a wide variety of {\em preferential attachment models} (PAMs).

By preferential attachment models we denote a class of random graphs with a common dynamics: At every time step, a new vertex appears in the graph, and it connects {to} $m\geq1$ existing vertices, with probability proportional to a function of the degrees \FC{of the vertices}. In other words, when vertex $n\in\N$ appears, all of its edges connects to vertex $i\leq n$ with probability
\eqn{
	\label{for:heur:PAfunction}
	\pr(n\rightsquigarrow  i \mid \mathrm{PA}_{n-1}) \propto f(d_i(n-1)),
}	
where \FC{$\PA_{n}$ is the preferential attachment graph with $n$ vertices,} $d_i(n-1)$ denotes the degree of vertex $i$ in the graph $\PA_{n-1}$, and $f$ is some \FC{preferential attachment} function. We {thus} in fact {consider a whole} PA class of random graphs since every function $f$ defines a different model.
The original Barab\'asi-Albert model is retrieved with $f(k) = k$. The literature often considers the so-called {\em affine} PAM, where $f(k) = k+\delta$, for some constant $\delta>-m$.

The constant $\delta$ allows for flexibility in the graph structure. In fact, the power-law exponent of the degree distribution is given by $\tau= 3+\delta/m$ \cite{BRST01, Der2009,vdH1}, and in general, for $m\geq 2$, the typical distance and the diameter are of order $\log\log n$ when $\tau\in(2,3)$, while they are of order $\log n$ when $\tau>3$. When $\tau=3$, distances and diameter are of order $\log n/\log\log n$ {instead} \cite{BolRio04b,CarGarHof,DSMCM,DSvdH}.

\begin{figure}
	\centering
	\includegraphics[scale=0.5]{Chap1_Intro/Chap1figs/PA_ex.png}
	\caption{Realisation of preferential attachment model on \(100\) vertices}	
\end{figure}


In {PAMs}, the degree of a vertex increases over time and higher degree vertices are prone to attract the edges incident to new vertices, increasing their degrees even further. In literature, this is sometimes referred {to as} \textit{rich-get-richer} effect. The models where the vertex degrees are determined by a \textit{weight} associated to it are sometimes called \textit{rich-by-birth} {models}. 

In \cite{DEH09}, the authors have considered a model incorporating both of these effects. The model is a {PAM} with random {out-degrees}, i.e., every vertex joins the existing network with a random number of edges that it connects to the existing vertices preferentially to their degrees at that time, as done in usual preferential attachment models. Here, the authors have shown that this system also shows the power-law degree distribution. {Jordan \cite{jordan06} considered} a special case of this particular model to analyze their results on degree distribution of the random graph. 

Cooper and Frieze \cite{cooper2003} have shown  that a further generalised version of this PAM also {has a} power-law degree distribution. Since most real-life networks are dynamic in nature and have power-law degrees, the PAM is often used to model them. However, in such networks it is never the case that every vertex joins with exactly the same out-degree, and instead i.i.d.\ out-degrees are more realistic. Gao and van der Vaart \cite{GV17} have shown that the maximum likelihood estimator of the fitness parameter $\delta$ of PAM with random out-degrees is asymptotically normal and has asymptotically minimal variance.
There have been further generalisations by allowing younger vertices to have higher degrees in PAMs through a random {\em fitness} parameter. More precisely, individual fitness factors \((\eta_i)_{i\geq 1}\) can be assigned to vertices, resulting in the probabilities in \eqref{for:heur:PAfunction} being proportional to \(\eta_i f(d_i(n-1))\), thus yielding PAMs \emph{with multiplicative fitness}, or proportional to \(d_i(n-1) + \eta_i\), giving rise to \emph{additive fitness} \cite{B07,Bianconi,Borgs,der16,der2014}. Usually, \((\eta_i)_{i\geq 1}\) is chosen as a sequence of i.i.d.\ random variables.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Model definition}\label{chap:intro:sec:model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{Several versions} of preferential attachment models are available in the literature. We generalize these definitions to the case of a random initial {number of edges that connect to the already available graph. We refer to these edge numbers as {\em out-degrees}, even though we consider our model to be {\em undirected.}} 
%Let $(M,m_i)_{i\ge 3}$ be {a sequence of i.i.d.\ $\N$-valued random variables} with finite $p$-th moment for some $p>1$, and $\delta >-{\infsupp}(M)$ be a fixed real number, {where $\operatorname{supp}(M)$ denotes the support of the random variable $M$}. 
Let $(m_i)_{i\ge 3}$ be {a sequence of i.i.d.\ copies of $M$ which is a $\N$-valued random variable} with finite $p$-th moment for some $p>1$, and $\delta >-{\infsupp}(M)$ be a fixed real number, {where $\operatorname{supp}(M)$ denotes the support of the random variable $M$}.
In our models, every new vertex $v$ joins the graph with $m_v$ many edges incident to it. 
%{In the classical preferential attachment models, instead,} every new vertex comes with a {\em fixed} number of edges incident to it. 
In case of self-loops, degree of the new vertex increases by $2$.
{Thus,} we can consider the existing models as a degenerate case of ours. Define $m_1=m_2=1$, $\boldsymbol{m}=(m_1,m_2,m_3,\ldots)$ and
\[
m_{[l]} = \sum\limits_{i\leq l} m_i.
\]
To describe the {edge-connection probabilities} and to simplify our calculations, we {frequently work with the conditional law given $\boldsymbol{m}=(m_i)_{i\ge 1}$}. %Let $\boldsymbol{m}$ be the sigma-field generated by $(m_i)_{i\geq 1}$. 
The conditional measure is denoted by $\prob_m$, i.e., for any event $\mathcal{E}$,
\eqn{\label{eq:conditional_measure:M} \prob_m(\mathcal{E})= \prob\left( \left. \mathcal{E} \right| \boldsymbol{m} \right).}
{Conditionally} on $\boldsymbol{m}$, we define some {versions of the preferential attachment models,} special cases of which {are} equivalent to the models~(a-g) described in \cite{GarThe}. We consider the initial graph to be $G_0$ with $2$ vertices with degree $a_1$ and $a_2$, respectively. {Throughout the remainder of this thesis, we fix}  $\delta>-\infsupp(M)$.
%\smallskip
%----------------------------------------------------------------------------------------------
\paragraph{\bf Model (A)} {This is} the generalized version of \cite[Model (a)]{vdH1}. Conditionally on $\boldsymbol{m}$, for $v\in\N$ and $j=1,\ldots,m_v$, the attachment probabilities are given by
\eqn{
	\label{eq:edge_connecting:model(rs):2}
	\prob_m\left(\left. v\overset{j}{\rightsquigarrow} u\right| \PArs_{v,j-1}(\boldsymbol{m},\delta) \right) = \begin{cases}
		\frac{d_u(v,j-1)+\delta}{c_{v,j}}\qquad\qquad \mbox{ for $v>u$},\\
		\frac{d_u(v,j-1)+1+\frac{j}{m_u}\delta}{c_{v,j}}\qquad \mbox{ for $v=u$},
	\end{cases}
}
where $v\overset{j}{\rightsquigarrow} u$ denotes that vertex $v$ connects to $u$ with its $j$-th edge, $\PArs_{v,j}(\boldsymbol{m},\delta)$ denotes the graph with $v$ vertices, \FC{with} the $v$-th vertex \FC{having} $j$ out-edges, and $d_u(v,j)$ denotes the degree of vertex $u$ in $\PArs_{v,j}(\boldsymbol{m},\delta)$. We identify $\PArs_{v+1,0}(\boldsymbol{m},\delta)$ with $\PArs_{v,m_v}(\boldsymbol{m},\delta)$. The normalizing constant $c_{v,j}$ in \eqref{eq:edge_connecting:model(rs):2} equals
\eqn{\label{eq:normali}
	c_{v,j} := a_{[2]}+2\left( m_{[v-1]}+j-2 \right) - 1+ (v-1)\delta + \frac{j}{m_v}\delta \, ,
}
where $a_{[2]}=a_1+a_2$. We denote the above model by $\PArs_v(\boldsymbol{m},\delta)$. If we consider $M$ as a degenerate distribution {that is equal to $m$ a.s.}, then $\PArs_v(\boldsymbol{m},\delta)$ is essentially equivalent to $\PA_v^{\sss ({m},\delta)}(a)$ defined in \cite{vdH2}. $\PA_v^{({m,0})}(a)$ was {informally introduced in \cite{albert1999} and first studied rigorously in \cite{BolRio04b}.}
Later the model for general $\delta$ was described in \cite{ABrB}.
\smallskip
%--------------------------------------------------------------------------------------------------
\paragraph{\bf Model (B)} {This is} the generalized version of \cite[Model (b)]{vdH1}. Conditionally on $\boldsymbol{m}$, the attachment probabilities are given by
\eqn{\label{eq:edge_connecting:model(rt):2}
	\prob_m\left(\left. v\overset{j}{\rightsquigarrow} u\right| \PArt_{v,j-1}(\boldsymbol{m},\delta) \right) = \begin{cases}
		\frac{d_u(v,j-1)+\delta}{c_{v,j}}\qquad\qquad \mbox{ for $v>u$},\\
		\frac{d_u(v,j-1)+\frac{(j-1)}{m_u}\delta}{c_{v,j}}\qquad \mbox{ for $v=u$},
\end{cases}}
where again $\PArt_{v,j}(\boldsymbol{m},\delta)$ denotes the graph with $v$ vertices, \FC{with} the $v$-th vertex \FC{having} $j$ out-edges, and $d_u(v,j)$ denotes the degree of vertex $u$ in $\PArt_{v,j}(\boldsymbol{m},\delta)$. We identify $\PArt_{v+1,0}(\boldsymbol{m},\delta)$ with $\PArt_{v,m_v}(\boldsymbol{m},\delta)$. The normalizing constant $c_{v,j}$ in \eqref{eq:edge_connecting:model(rt):2} now equals
\[
c_{v,j} = a_{[2]}+2\left( m_{[v-1]}+j-3 \right) +(v-1)\delta + \frac{(j-1)}{m_v}\delta \,.
\]
We denote the above model by $\PArt_v(\boldsymbol{m},\delta)$. For $M$ a degenerate distribution {which is equal to $m$ a.s.}, we obtain $\PA_v^{\sss ({m},\delta)}(b)$ described in \cite{vdH2} from $\PArt_v(\boldsymbol{m},\delta)$.
%\smallskip
\FC{\begin{remark}[Difference between models (A) and (B)]
		\rm{From the definition of the models (A) and (B), the models are different in that the first edge from every new vertex can create a self-loop in model (A) but not in model (B). Note that the edge probabilities are different for all $j$.}\hfill$\blacksquare$
\end{remark}}
%--------------------------------------------------------------------------------------------------
\paragraph{\bf Model (D)} This model is the generalized {version} of the sequential model described in \cite{BergerBorgs}. We start with a fixed graph $G_0$ of size $2$ and degrees $a_1$ and $a_2$, respectively. Denote the graph {by} $\PAri_{v}(\boldsymbol{m},\delta)$ when {the graph has $v$ vertices.}

For $v\geq 3$, vertex $v$ enters the system with $m_v$ many out-edges {whose} edge-connection probabilities are given by
\eqn{\label{sec:model:eq:1}
	\prob_m\left(\left. v\overset{j}{\rightsquigarrow} u \right| \PAri_{v,j-1} \right) = 
	\frac{d_u(v,j-1)+\delta}{c_{v,j}}\quad \text{for}\quad v>u,
}
where $\PAri_{v,j}(\boldsymbol{m},\delta)$ denotes the graph with $v$ vertices, \FC{with} the $v$-th vertex \FC{having} $j$ out-edges, $d_u(v,j)$ is the degree of the vertex $u$ in the graph $\PAri_{v,j}$, and
\begin{equation*}
	c_{v,j}= a_{[2]}+2\left( m_{[v-1]}-2 \right)+(j-1) + (v-1)\delta\,.
\end{equation*}
Again we identify $\PAri_{v+1,0}(\boldsymbol{m},\delta)$ with $\PAri_{v,m_v}(\boldsymbol{m},\delta)$. For $M$ a degenerate random variable {that is equal to $m$ a.s.}, we obtain $\PA_v^{\sss ({m},\delta)}(d)$, {as} described in \cite{vdH2}.
%\smallskip
%------------------------------------------------------------------------------------------------------
{\paragraph{\bf Model (E)} This model is the independent model proposed {by Berger et al.\ in \cite{DEH09}}. We start with the same initial graph $G_0$. We name the graph $\PArf_{v}(\boldsymbol{m},\delta)$ when there are $v$ vertices in the graph. Conditionally on $\boldsymbol{m},$ every new vertex $v$ is added to the graph with $m_v$ many {out-edges}. Every {out-}edge $j\in[m_v]$ from $v$ connects to the vertex $u\in[v-1]$ independently with the {probabilities}
	\eqn{\label{eq:model:f:1}
		\prob_m\left( \left.v\overset{j}{\rightsquigarrow}u\right|\PArf_{v-1}(\boldsymbol{m},\delta) \right) = \frac{d_u(v-1)+\delta}{a_{[2]}+2(m_{[v-1]}-2)+(v-1)\delta},}
	where $d_{u}(v-1)$ is the degree of the vertex $u$ in $\PArf_{v-1}$. Note that the intermediate degree updates are not there in this graph. Similarly as {in} model (D), no self-loops are allowed here.}
%\smallskip

\paragraph{\bf Model (F)} The independent model does not allow for self-loops, but multiple {edges} between two vertices {may still occur}. {Such multigraphs are, in many applications, unrealistic, and we next propose a model where the graphs obtained are {\em simple}, i.e., without self-loops and multiple edges.} Model (F) is a variation of the independent model where the new vertices connect to the existing vertices in the graph independently {but {\em without replacement}} and the edge-connection probabilities are {similar to} \eqref{eq:model:f:1}. Indeed, for $j\geq 2$, the normalization factor changes a little due to the fact that vertices that have already appeared as neighbours are now forbidden. The degenerate case of our PAM, i.e., with fixed out-degree, is studied in \cite{basu2014} for analyzing the largest connected component in the strong friendship subgraph of evolving online social networks.

%\RvdH{Refer to paper that was brought to our attention}
%\RR{done!}
\begin{remark}[{The missing model (c)}]
	{\rm There is a description of model (c) in \cite[Section 8.2]{vdH1}, which {reduces to model (a), so we refrain from discussing it further in this Chapter}. %Hence we also avoid {to discuss} model (c).
	}\hfill$\blacksquare$ 
\end{remark}


==> Chap3_PU_Graph/Chap3figs/alpha-glep.tex <==
   
\begin{tikzpicture}
  \draw[->, very thick] (-0.1, 0) -- (10, 0) node[right] {$x$};
  \draw[->,very thick] (0, -0.1) -- (0, 6.3) node[left] {$y$};
  \node at (-0.2,-0.2) {$0$};
  
  \draw[->, Neonpink][line width=1.3] (1,6.3) -- (1,5) -- (1,5) -- (2,5) -- (2,5) -- (2,3) -- (2,3) -- (4,3) -- (4,3) -- (4,1) -- (4,1) -- (8,1) -- (8,1) -- (8,0.5) -- (8,0.5) -- (9,0.5) ;
  \node at (9.675,0.4) {$\alpha=2$};
  
  \draw[->, Neongreen][line width=1.1]  ( 1 , 5.5 )--   ( 1.5 , 5.5 ) -- ( 1.5 , 5.5 )--   ( 1.5 , 5.5 ) -- ( 1.5 , 5.5 )  -- ( 2 , 5.5 ) -- ( 2 , 5.5 ) --  ( 2 , 3.598 ) -- ( 2 , 3.598 )  -- ( 2.5 , 3.598 ) -- ( 2.5 , 3.598 )  -- ( 2.5 , 3.598 ) -- ( 2.5 , 3.598 ) --  ( 3 , 3.598 )--  ( 3 , 3.598 ) --  ( 3 , 3.598 ) -- ( 3 , 3.598 ) --  ( 3.5 , 3.598 ) -- ( 3.5 , 3.598 ) --  ( 3.5 , 3.387 ) -- ( 3.5 , 3.387 ) --  ( 4 , 3.387 ) -- ( 4 , 3.387 )  -- ( 4 , 1.442 ) -- ( 4 , 1.442 )  -- ( 4.5 , 1.442 ) -- ( 4.5 , 1.442 ) --  ( 4.5 , 1.442 )--  ( 4.5 , 1.442 ) --  ( 5 , 1.442 ) -- ( 5 , 1.442 ) --  ( 5 , 1.442 ) -- ( 5 , 1.442 )--   ( 5.5 , 1.442 )--  ( 5.5 , 1.442 ) --  ( 5.5 , 1.442 ) -- ( 5.5 , 1.442 )--   ( 6 , 1.442 ) -- ( 6 , 1.442 )  -- ( 6 , 1.442 )--  ( 6 , 1.442 ) --  ( 6.5 , 1.442 ) -- ( 6.5 , 1.442 ) --  ( 6.5 , 1.442 )--  ( 6.5 , 1.442 ) --  ( 7 , 1.442 )--  ( 7 , 1.442 ) --  ( 7 , 1.442 ) -- ( 7 , 1.442 ) --  ( 7.5 , 1.442 )--  ( 7.5 , 1.442 ) --  ( 7.5 , 1.442 ) -- ( 7.5 , 1.442 ) --  ( 8 , 1.442 ) -- ( 8 , 1.442 )--   ( 8 , 0.687 )  --( 8 , 0.687 ) --  ( 8.5 , 0.687 ) -- ( 8.5 , 0.687 ) --  ( 8.5 , 0.687 ) -- ( 8.5 , 0.687 )  -- ( 9 , 0.687 );
    \node at (9.8,0.787) {$\alpha=1.7$};

  
  \draw[->, Neonblue][line width=0.9]
  (1,6.3)--( 1 , 6 )  -- ( 1.5 , 6 )-- ( 1.5 , 6 )   --( 1.5 , 6 ) -- ( 1.5 , 6 ) --  ( 2 , 6 ) -- ( 2 , 6 ) --  ( 2 , 4.874 )--  ( 2 , 4.874 )  -- ( 2.5 , 4.874 ) -- ( 2.5 , 4.874 )--  ( 2.5 , 4.874 ) -- ( 2.5 , 4.874 ) --  ( 3 , 4.874 )--  ( 3 , 4.874 ) --  ( 3 , 4.593 ) -- ( 3 , 4.593 )  -- ( 3.5 , 4.593 ) -- ( 3.5 , 4.593 ) --  ( 3.5 , 4.159 )-- ( 3.5 , 4.159 ) --  ( 4 , 4.159 )  --( 4 , 4.159 ) --  ( 4 , 2.712 )--  ( 4 , 2.712 ) --  ( 4.5 , 2.712 ) -- ( 4.5 , 2.712 )  -- ( 4.5 , 2.712 )  --( 4.5 , 2.712 )  -- ( 5 , 2.712 )  ( 5 , 2.712 ) --  ( 5 , 2.712 ) -- ( 5 , 2.712 )  -- ( 5.5 , 2.712 ) -- ( 5.5 , 2.712 ) --  ( 5.5 , 2.475 ) -- ( 5.5 , 2.475 ) --  ( 6 , 2.475 )--  ( 6 , 2.475 )   --( 6 , 2.475 ) -- ( 6 , 2.475 )  -- ( 6.5 , 2.475 ) -- ( 6.5 , 2.475 ) --  ( 6.5 , 2.322 ) -- ( 6.5 , 2.322 ) --  ( 7 , 2.322 ) -- ( 7 , 2.322 )  -- ( 7 , 2.322 )--  ( 7 , 2.322 )  -- ( 7.5 , 2.322 ) -- ( 7.5 , 2.322 )  -- ( 7.5 , 2.322 ) -- ( 7.5 , 2.322 )--   ( 8 , 2.322 ) -- ( 8 , 2.322 )  -- ( 8 , 1.465 ) -- ( 8 , 1.465 )  -- ( 8.5 , 1.465 ) -- ( 8.5 , 1.465 )  -- ( 8.5 , 1.465 )--  ( 8.5 , 1.465 ) --  ( 9 , 1.465 );
  \node at (9.8,1.465) {$\alpha=1.3$};
  
   \foreach \Point in {(1,5),(1.5,6.2), (2,3), (2.5,6), (3,4), (3.5,3.3), (4,1), (4.5,6), (5,4), (5.5,2), (6,5), (6.5,2), (7,3.3), (7.5,3), (8,0.5), (8.5,2), (8.8,2.6), (8.7,4)}{
    \node at \Point {\textbullet};
  }
  
\end{tikzpicture}


==> Chap3_PU_Graph/Chap3figs/alphaLEPgeq1.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da18822060405945962] 
\draw    (51.2,219.3) -- (51.2,10) ;
\draw [shift={(51.2,7)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7239860136829701] 
\draw    (29.87,199.4) -- (452.2,200.46) ;
\draw [shift={(455.2,200.47)}, rotate = 180.14] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da15061569369102368] 
\draw    (100.53,193.13) -- (100.53,205.13) ;
%Straight Lines [id:da3522689736325253] 
\draw    (150.13,193.73) -- (150.13,205.73) ;
%Straight Lines [id:da6026212061771374] 
\draw    (200.53,193.93) -- (200.53,205.93) ;
%Straight Lines [id:da5721333585606583] 
\draw    (250.53,193.93) -- (250.53,205.93) ;
%Straight Lines [id:da5820239080249348] 
\draw    (300.13,193.93) -- (300.13,205.93) ;
%Straight Lines [id:da4076775067321772] 
\draw    (350.13,193.93) -- (350.13,205.93) ;
%Straight Lines [id:da46847183587733476] 
\draw    (55.8,50.03) -- (45.2,50.05) ;
%Straight Lines [id:da203148923728232] 
\draw    (55.8,100.03) -- (45.2,100.05) ;
%Straight Lines [id:da9807979735513521] 
\draw    (55.8,150.18) -- (45.2,150.2) ;
%Straight Lines [id:da8751705938700838] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (28,149.33) -- (439.2,151) ;
%Straight Lines [id:da10631841197835556] 
\draw [color={rgb, 255:red, 255; green, 95; blue, 31 }  ,draw opacity=1 ][line width=1.5]    (51.33,132) -- (133.2,131.93) ;
%Straight Lines [id:da18477268012702996] 
\draw [color={rgb, 255:red, 255; green, 95; blue, 31 }  ,draw opacity=1 ][line width=1.5]    (133.2,181.2) -- (133.2,131.93) ;
%Straight Lines [id:da06576532342004704] 
\draw [color={rgb, 255:red, 255; green, 95; blue, 31 }  ,draw opacity=1 ][line width=1.5]    (133.2,181.2) -- (205.2,181.2) ;
%Straight Lines [id:da033091389621956235] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]    (133.7,149.7) -- (171.7,149.8) ;
%Straight Lines [id:da26710706798299877] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]    (171.2,172.7) -- (171.7,149.8) ;
%Straight Lines [id:da47620899957728846] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (56.83,71) -- (94.2,71.2) ;
%Straight Lines [id:da11368030620224556] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (94.2,102.97) -- (94.2,71.2) ;
%Straight Lines [id:da41355419772378577] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (94.2,102.97) -- (194.7,103.3) ;
%Straight Lines [id:da28335117858385006] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (56.83,71) -- (57.2,7.5) ;
%Straight Lines [id:da8695923576693758] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (194.7,135.07) -- (194.7,103.3) ;
%Straight Lines [id:da258354259933228] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (194.7,135.07) -- (295.2,135.4) ;
%Straight Lines [id:da1650372711600201] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (295.2,167.17) -- (295.2,135.4) ;
%Straight Lines [id:da2813981785179207] 
\draw    (52.67,242.71) -- (89.34,242.46) -- (112.02,242.3) -- (289.7,241.71) ;
\draw [shift={(292.7,241.7)}, rotate = 179.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(49.67,242.73)}, rotate = 359.6] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6034421010501376] 
\draw    (136.2,261.2) -- (148.8,261.2) -- (167.2,261.2) ;
\draw [shift={(170.2,261.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(133.2,261.2)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8750981327404972] 
\draw    (54.09,260.02) -- (98.69,260.24) -- (130.2,261.12) ;
\draw [shift={(133.2,261.2)}, rotate = 181.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(51.09,260)}, rotate = 0.29] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (95.33,213.93) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1$};
% Text Node
\draw (144.93,214.53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 2$};
% Text Node
\draw (195.33,214.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 3$};
% Text Node
\draw (245.33,214.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 4$};
% Text Node
\draw (295.73,214.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 5$};
% Text Node
\draw (344.93,214.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 6$};
% Text Node
\draw (31.9,41.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 3$};
% Text Node
\draw (31.9,91.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 2$};
% Text Node
\draw (31.9,141.65) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1$};
% Text Node
\draw (32.9,213.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 0$};
% Text Node
\draw (21.27,120.2) node [anchor=north west][inner sep=0.75pt]    {$V_{0}$};
% Text Node
\draw (176.6,149.7) node [anchor=north west][inner sep=0.75pt]    {$\tilde{V}_{N( t)}( \eta )$};
% Text Node
\draw (269.23,242.82) node [anchor=north west][inner sep=0.75pt]    {$\tau _{1}$};
% Text Node
\draw (142.83,263.07) node [anchor=north west][inner sep=0.75pt]    {$\tau _{2}$};
% Text Node
\draw (81.09,261.4) node [anchor=north west][inner sep=0.75pt]    {$n_{1}$};
% Text Node
\draw (154.43,77.2) node [anchor=north west][inner sep=0.75pt]    {$L_{\hat{\alpha }}( t)$};


\end{tikzpicture}

==> Chap3_PU_Graph/Chap3figs/alphaLEPleq1.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da006915578794734145] 
\draw    (71.93,219.63) -- (71.93,10.33) ;
\draw [shift={(71.93,7.33)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da37965598201185213] 
\draw    (50.6,199.73) -- (472.93,200.79) ;
\draw [shift={(475.93,200.8)}, rotate = 180.14] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7434248768936242] 
\draw    (121.27,193.47) -- (121.27,205.47) ;
%Straight Lines [id:da537182371547849] 
\draw    (170.87,194.07) -- (170.87,206.07) ;
%Straight Lines [id:da4276888792678648] 
\draw    (221.27,194.27) -- (221.27,206.27) ;
%Straight Lines [id:da7640358069581787] 
\draw    (271.27,194.27) -- (271.27,206.27) ;
%Straight Lines [id:da31790329293605235] 
\draw    (320.87,194.27) -- (320.87,206.27) ;
%Straight Lines [id:da37207100433720797] 
\draw    (370.87,194.27) -- (370.87,206.27) ;
%Straight Lines [id:da08642197784104577] 
\draw    (76.53,50.36) -- (65.93,50.38) ;
%Straight Lines [id:da16797642520293543] 
\draw    (76.53,100.36) -- (65.93,100.38) ;
%Straight Lines [id:da5781200746440842] 
\draw    (76.53,150.51) -- (65.93,150.53) ;
%Straight Lines [id:da7495713267064288] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (48.73,149.67) -- (459.93,151.33) ;
%Straight Lines [id:da12861014015069405] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]    (70.07,164.33) -- (151.93,164.27) ;
%Straight Lines [id:da5576529585767369] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]    (152.2,182.07) -- (151.93,164.27) ;
%Straight Lines [id:da07533952473002925] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]    (152.2,182.07) -- (224.2,182.07) ;
%Straight Lines [id:da528735054104428] 
\draw [color={rgb, 255:red, 255; green, 16; blue, 240 }  ,draw opacity=1 ][line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (151.93,164.27) -- (289.67,164.13) ;
%Straight Lines [id:da8587002170684253] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (77.57,71.33) -- (114.93,71.53) ;
%Straight Lines [id:da9694480885645949] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (114.93,103.3) -- (114.93,71.53) ;
%Straight Lines [id:da48590366523836437] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (114.93,103.3) -- (215.43,103.63) ;
%Straight Lines [id:da6782789425531288] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (77.57,71.33) -- (77.93,7.83) ;
%Straight Lines [id:da11926541445401795] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (215.43,135.4) -- (215.43,103.63) ;
%Straight Lines [id:da9339245987328786] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (215.43,135.4) -- (315.93,135.73) ;
%Straight Lines [id:da14950631179806684] 
\draw [color={rgb, 255:red, 15; green, 255; blue, 80 }  ,draw opacity=1 ][line width=1.5]    (315.93,167.5) -- (315.93,135.73) ;
%Straight Lines [id:da07308910596150042] 
\draw    (73.4,243.05) -- (110.07,242.79) -- (132.75,242.63) -- (310.43,242.04) ;
\draw [shift={(313.43,242.03)}, rotate = 179.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(70.4,243.07)}, rotate = 359.6] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9049153120056541] 
\draw    (74.43,260.53) -- (87.03,260.53) -- (105.2,260.53) -- (149.2,260.97) ;
\draw [shift={(152.2,261)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(71.43,260.53)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (116.07,214.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1$};
% Text Node
\draw (165.67,214.87) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 2$};
% Text Node
\draw (216.07,215.07) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 3$};
% Text Node
\draw (266.07,215.07) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 4$};
% Text Node
\draw (316.47,215.07) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 5$};
% Text Node
\draw (365.67,215.07) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 6$};
% Text Node
\draw (52.63,41.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 3$};
% Text Node
\draw (52.63,91.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 2$};
% Text Node
\draw (52.63,141.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1$};
% Text Node
\draw (53.63,214.08) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 0$};
% Text Node
\draw (227.67,166.03) node [anchor=north west][inner sep=0.75pt]    {$\tilde{V}_{N( t)}( \eta )$};
% Text Node
\draw (289.97,243.15) node [anchor=north west][inner sep=0.75pt]    {$\tau _{1}$};
% Text Node
\draw (127.57,262.9) node [anchor=north west][inner sep=0.75pt]    {$\tau _{2}$};
% Text Node
\draw (175.17,77.53) node [anchor=north west][inner sep=0.75pt]    {$L_{\hat{\alpha }}( t)$};
% Text Node
\draw (26.8,158.33) node [anchor=north west][inner sep=0.75pt]    {$\tilde{V}_{0}( \eta )$};


\end{tikzpicture}

==> Chap4_Convergence/chap4_cupling.tex <==
\section{Coupling between models (E), (F) and (D)}
\label{chap:convergence:sec:coupling}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we prove that models (D), (E) and (F) have the same local limit.
We do this by showing that for any fixed $r\geq 1$, we can couple models (D), (E) and (F) in such a way that whp, the $r$-neighbourhoods of a uniformly chosen vertex in \FC{all these} models are identical. 

\FC{We follow the same coupling used in \cite{BergerBorgs} with proper modifications as required for our models. In the coupling argument we work on the high-probability event $\mathcal{E}=\mathcal{E}_m\cap \mathcal{E}_{\sss \hat{\chi},\psi},$ where $\mathcal{E}_m$ and $\mathcal{E}_{\sss \hat{\chi},\psi}$ are $\{\boldsymbol{m}\}$ and $\{\boldsymbol{m,\psi}\}$ measurable events respectively. In $\mathcal{E}_m$, following regularity properties hold true:
	\begin{enumerate}
		\item $m_v\leq v^{1-\varrho/2}$ for all {$v>K$ for some $K\in\N$;}\label{reg:3}
		%\item $\{ \hat{\chi}_v \}_{v\geq 1}$ has uniformly bounded $(1+p)$-th moment;\label{reg:1} %and $\E_m\left[ \hat{\chi}_v \right] = m_v+\delta.$
		\item {for $\eta^\prime=\eta(\varepsilon/8,2r)$,} there exists a $c_0$ such that \label{reg:4}
		\[
		\frac{1}{n}\sum\limits_{u\geq \eta^\prime n}m_u\left( \frac{u}{n} \right)^{-\chi} \leq c_0;
		\]
	\end{enumerate}
	whereas in $\mathcal{E}_{\sss \hat{\chi},\psi}$, the bounds on the attachment probabilities in Lemma~\ref{lem:bound:attachment_probability} hold true.
	{In Section~\ref{subsec-pos-conc-Beta-gamma-coupling}, we have proved that $\mathcal{E}_{\sss \hat{\chi},\psi}$ is a high probability event and from \eqref{for:lem:NFE:main:3}, substituting $a_\omega$ by $\eta^\prime$, we can prove that \eqref{reg:4} is also a high probability event. By Proposition~\ref{prop:Betagamma:coupling:CPU}~(i), \eqref{reg:3} follows whp from the Borel-Cantelli Lemma proving $\mathcal{E}_m$ also a high probability event. Therefore $\mathcal{E}$ is indeed a high probability event} and $\prob(\mathcal{E})>1-{\varepsilon/4}$.}
%\RR{I have added the events explicitly.}
%\RvdH{Part (3) is not quantitative. Can we make this quantitative by making claims on the neighbourhoods in model (D)? Check where we actually use (3).}
%Let $\prob_\mathcal{E}$ and $\E_\mathcal{E}$ denote the law and expectation conditionally on this high probability event. From now on, we work on this good event  $\mathcal{E}$.

The proof for models (E) and (F) are highly similar. \arxiversion{Thus, in this section we provide the coupling argument for model (E) in detail, and state the adaptations for model (F).}
%Since $m_i$ have $(1+p)$-th moment finite, by Borel-Cantelli lemma, with probability at least $1-\varepsilon,$
%\[
%    m_l\leq l,~\forall~ l>\eta n.
%\]


{For} all $j\in[m_n],$ the conditional edge-connection probability for model (E) is given by
\eqn{\label{edge:probability:F}
	\begin{split}
		\prob_m\left( n\overset{j}{\rightsquigarrow} v\left| \PArf_{n-1}(\boldsymbol{m},\delta)  \right.\right)=~\frac{d_v(n-1)+\delta}{a_{[2]}+2\left( m_{[n-1]}-2 \right)+(n-1)\delta}\,.
\end{split}}
We aim to couple $\PArf_n(\boldsymbol{m},\delta)$ with $\PAri_n(\boldsymbol{m},\delta)$.
Let $V=\{ 1,2,\ldots \}$ be the vertices of the preferential attachment model. For $1\neq n\in V$ and $i\in [m_n]$, $e_n^i$ and $f_n^i$ denote the vertices in $[n-1]$ to which vertex $n$ connects with its $i$-th edge in models (D) and (E), {respectively}. Denote
\eqn{
	\begin{split}
		{\mathbf{e}_n}=\left\{ e_n^i \right\}_{i\in[m_n]}\qquad \text{and}\qquad \mathbf{f}_n=\left\{ f_n^i \right\}_{i\in[m_n]}\,.
\end{split}}
Since we start with the same initial graph $G_0,~\mathbf{e}_2=\mathbf{f}_2$. 
{Conditionally} on $\boldsymbol{m}$, \(\{{\bf{e}}_{\ell}\}_{\ell<n}\), and \( \{{\bf{e}}_n^{i}\}_{i<j} \), let \({\bf{e}}_n^{j}\) have distribution \(D_1^{\sss(n,j)}\), and conditionally on $\{\mathbf{f}_l\}_{l<n},~\mathbf{f}_n^j$ have distribution $D_2^{\sss(n,j)}$. Let \(D^{(n,j)}\) be a coupling of $D_1^{\sss(n,j)}$ and $D_2^{\sss(n,j)}$ that minimizes the total variation distance. Then, we choose $\mathbf{e}_n^{j}$ and $\mathbf{f}_n^{j}$ according to $D^{\sss(n)}$. This provides us with a coupling between models (D) and (E).
%let $\mathbf{e}_n$ have distribution $D_1^{\sss(n)}$ and, conditionally on $\{\mathbf{f}_l\}_{l<n},~\mathbf{f}_n$ have distribution $D_2^{\sss(n)}$. Let $D^{\sss(n)}$ be a coupling of $D_1^{\sss(n)}$ and $D_2^{\sss(n)}$ that minimizes the total variation distance. Then, we choose $\mathbf{e}_n$ and $\mathbf{f}_n$ according to $D^{\sss(n)}$. This provides us with a coupling between models (D) and (E).
%-------------------------------------------------------
\begin{Proposition}[Coupling between models (D) and (E)]{\label{prop:coupling:D:E}}
	Let $(G_n)_{n\geq 2}$ and $(G_n^\prime)_{n\geq 2}$ be the sequences of preferential attachment graphs of models (D) and (E), respectively. Fix $\varepsilon>0$ and $r\in\N$. Then, there exist {a coupling $(\hat{G}_n, \hat{G}_n^\prime)_{n\geq 1}$ and $n_0\in\N$} (possibly depending on $\varepsilon$ and $r$) such that for all $n>n_0,$ with probability at least $1-\varepsilon,$ the $r$-neighbourhoods of a randomly chosen vertex $o_n\in[n]$ are the same in both $G_n$ and $G_n^\prime$.
	%Similar coupling results holds for model (F) as well.
\end{Proposition}
%\RvdH{Have you actually described the coupling anywhere?}
%\RR{The coupling just before the proposition?}
%------------------------------------------------------
\begin{proof}[Proof of Theorem~\ref{theorem:PArs} for model (E)]
	\chRounak{Subject to Proposition~\ref{prop:coupling:D:E}, the proof of Theorem~\ref{theorem:PArs} follows immediately. In Proposition~\ref{prop:coupling:D:E}, we proved that for any fixed $r \geq 1$, with high probability, the $r$-neighbourhoods of a randomly chosen vertex in models (D) and (E) are the same. In Section~\ref{chap:convergence:sec:local_convergence}, we showed that the $r$-neighbourhood of a randomly chosen vertex in model (D) converges in probability to that of an $\RPPT(M,\delta)$. Therefore, the same result holds true for model (E) as well.
	}
\end{proof}
%------------------------------------------------------
{Now, we move on to prove Proposition~\ref{prop:coupling:D:E}. To simplify notation, below we write $(G_n)_{n\geq 2}$ and $(G_n^\prime)_{n\geq 2}$ for the coupled graph processes.} Fix $\varepsilon>0$ and $r\in\N$ and let $B_r(v)$ and $B_r^\prime(v)$ denote the $r$-neighbourhood of $v$ in $G_n$ and $G_n^\prime$, respectively. We {denote} the set of bad vertices $v$ for which $B_r(v)\neq B_r^\prime(v)$ {by}
\[
\mathcal{B}_{n,r}=\left\{ v\in[n]\colon B_r(v)\neq B_r^\prime(v) \right\}.
\]
Since $o_n$ is chosen uniformly from the set of vertices, the probability that $o_n$ is a bad vertex {equals} $\E\left({|\mathcal{B}_{n,r}|/n}\right)$. {Thus,} to prove Proposition~{\ref{prop:coupling:D:E}}, it is enough to show that $\E(|\mathcal{B}_{n,r}|)\leq \varepsilon n.$



{We} claim that for {$B_r(v)\neq B_r^\prime(v)$ to hold, there must be a vertex $u \in B_r(v)$ such that either $ e_{n^\prime}^i=u\neq f_{n^\prime}^i$ or $e_{n^\prime}^i\neq u=f_{n^\prime}^i$ for some $n^\prime>u$ and $i\in [m_{n^\prime}].$} To investigate these bad vertices, {we thus concentrate on the bad events}
\eqn{\label{eq:bad:events}
	A_{n^\prime}^{\sss(u)}=\left\{ \exists~ i\in[m_{n^\prime}]\colon e_{n^\prime}^i=u\neq f_{n^\prime}^i,~\text{or}~e_{n^\prime}^i\neq u= f_{n^\prime}^i \right\}\,.
}

Let us consider $A^{\sss(u)}=\bigcup\limits_{n\geq n^\prime>u} A_{n^\prime}^{\sss(u)}$, i.e., $A^{\sss(u)}$ is the event that at least one of the edges received by $u$ is different in $G_n$ and $G_n^\prime$. The $1$-neighbourhoods of vertex $v$ {are different} in both $G_n$ and $G_n^\prime$ precisely when  $A^{\sss(u)}$ happens for at least one of the $u\in B_1(v)$. Now inductively on $r$, it {is easy to show} that $B_r(v)=B_r^\prime(v)$ unless there exists a $u\in B_r(v)$ for which $A^{\sss(u)}$ holds true.
%\RvdH{Maybe use $u$ or $w$ instead of $v^\prime$?}
%\RR{I have changed this to $u$.}

%\FC{This is the same $\eta^\prime$ we have used in (\ref{reg:4}) for defining $\mathcal{E}$.}

The following lemma gives us a tool to bound the probabilities of the bad events:
%-------------------------------------------------------
\begin{Lemma}[Conditional control on bad events]\label{lem:conditional:control:bad_events}
	With the coupling {of models (E) and (D)} defined earlier in this section and fixing $v\geq \eta^\prime n,$ we define $A_n=A_n^{\sss(v)}$ to keep the notations simple. Then,
	\eqn{\label{lem:eq:conditional:control:bad_events}
		\prob\left( A_n\cap\mathcal{E}\left|\bigcap\limits_{h=v+1}^{n-1} A_h^c\cap \mathcal{E}\right. \right)=~o\left( {n^{-1}} \right)\,.}
	%The lemma holds true even if we consider the model (F) instead of model (E).
\end{Lemma}
%\RvdH{To be clear, is $A_h=A_h^{\sss(v)}$ here in the conditioning?}
%\RR{Yes. Only for proving this Lemma the above simplified notation is used.}
%-------------------------------------------------------
Lemma~\ref{lem:conditional:control:bad_events} implies {that}, conditionally on the event that there have not been any bad {events} till the $(n-1)$-st vertex joins the graph, the probability of the bad event taking place when the $n$-th vertex is joining the graph is $o({1/n}).$



We {first} provide the proof of Proposition~\ref{prop:coupling:D:E} subject to Lemma~\ref{lem:conditional:control:bad_events}, and then we prove Lemma~\ref{lem:conditional:control:bad_events}.
First we construct a set {$W_{n,r}$} of well-behaved vertices with the following properties:
\begin{itemize}
	\item[$\rhd$] for all $v\in W_{n,r}$, {$B_{2r}(v)$} has no more than $N$ vertices;
	\item[$\rhd$] the oldest vertex in $B_{2r}(v)$ is not older than $\eta^\prime n$.
\end{itemize}
By the proof of local convergence of model (D) and the regularity property of RPPT (Lemma~\ref{lem:RPPT:property}),
\eqn{\label{eq:nice:vertex:1}
	\E|W_{n,r}|\geq \left(1-\frac{\varepsilon}{2}\right)n.}
\begin{proof}[\bf Proof of Proposition~\ref{prop:coupling:D:E}]
	{To} prove the proposition, it is enough to show that
	\eqn{
		\label{eq:to:prove:prop:coupling:1}
		\E\left| W_{n,r}\cap \mathcal{B}_{n,r} \right|\leq {\varepsilon n/2}\,,}
	i.e., there are few well-behaved vertices that are bad. {To prove \eqref{eq:to:prove:prop:coupling:1}, we note that if} $v\in W_{n,r}\cap \mathcal{B}_{n,r},$ there must be a $u\in B_r(v)$ such that $A^{\sss(u)}$ is true. 
	Therefore,
	\eqn{\label{eq:to:prove:prop:coupling:2}
		\begin{split}
			\left| W_{n,r}\cap \mathcal{B}_{n,r} \right|=&\sum\limits_{v\in W_{n,r}}\one_{\{v\in \mathcal{B}_{n,r}\}}\leq \sum\limits_{v\in W_{n,r}}\sum\limits_{u\in B_{r}(v)}\one_{A^{\sss(u)}}\\
			=& \sum\limits_{u\in (\eta^\prime n,n]}\one_{A^{\sss(u)}}\sum\limits_{v\in B_r(u)}\one_{\{v\in W_{n,r}\}}.
	\end{split}}
	Note that the second sum in the RHS of \eqref{eq:to:prove:prop:coupling:2} produces $0$ if there is no well-behaved vertex in $B_r(u)$. Otherwise, the sum can be bounded by $\left|B_{r}(u)\right|$. Again $v \in B_r(u)$ implies that $u\in B_r(v)$ and $B_r(u)$ is a subset of $B_{2r}(v)$. If there is a well-behaved vertex in $B_r(u)$, we can bound $\left| B_r(u) \right|{\leq}N$ from the properties of the well-behaved vertices. Therefore the second sum on the RHS of \eqref{eq:to:prove:prop:coupling:2} can be uniformly bounded by $N$ for all vertices $u>\eta^\prime n$. Hence the cardinality of the well-behaved bad vertices can be further upper-bounded as
	\eqn{\label{eq:to:prove:prop:coupling:3}
		\left| W_{n,r}\cap \mathcal{B}_{n,r} \right|\leq N \sum\limits_{u\in (\eta^\prime n,n]}\one_{A^{\sss(u)}},}
	so that
	\eqn{\label{eq:to:prove:prop:coupling:3-1}
		\E \left| W_{n,r}\cap \mathcal{B}_{n,r} \right| \leq N\sum\limits_{u\in (\eta^\prime n,n]} \prob\left( A^{\sss(u)} \right).
	}
	{By} the control on the bad events obtained in Lemma~\ref{lem:conditional:control:bad_events} and $\Ecal$ defined earlier in Section~\ref{chap:convergence:sec:coupling},
	\eqan{\label{eq:to:prove:prop:coupling:4}
		%\begin{split}
		\prob\left( A^{\sss(u)} \right) = &\prob\Big( \bigcup\limits_{l=u+1}^{n}A^{\sss(u)}_{l}\cap\mathcal{E} \Big) + \prob (\mathcal{E}^c)\\
		= &\sum\limits_{l=u+1}^{n}\prob\Big( A^{\sss(u)}_l\cap \Big( \bigcap\limits_{h=u+1}^l \left(A^{\sss(u)}_h\right)^c \Big)\cap\mathcal{E} \Big) +\prob (\mathcal{E}^c) = o(1)+\varepsilon/4 .\nn
		%\end{split}
	}
	{Substituting} the bound {on} $\prob\left( A^{\sss(u)} \right)$ in \eqref{eq:to:prove:prop:coupling:3-1},
	\eqn{\label{eq:to:prove:prop:coupling:5}
		\E\left( \left| W_{n,r}\cap \mathcal{B}_{n,r} \right| \right) 
		= o(n)+{n\varepsilon/4},
	}
	which completes the proof of Proposition~\ref{prop:coupling:D:E} subject to Lemma~\ref{lem:conditional:control:bad_events}.
\end{proof}
{It remains to prove Lemma~\ref{lem:conditional:control:bad_events} about bad events, {for which} we need the following lemma:}
\begin{Lemma}[{Bounds on second moments of degrees in model (D)}]\label{Lem:auxiliary:control:bad_event}
	There exists $c_1>0$ such that for all $v\geq \eta^\prime n,$
	\eqn{\label{lem:eq:degree_bound}\E_{m}\left( d_{v}(n)^2\one_\mathcal{E} \right) \leq c_1m_v^2~.}
\end{Lemma} 
\begin{proof} By definition,
	\eqn{\label{for:claim:bad:event:1}
		d_v(n)=m_v+\sum\limits_{l=v+1}^n {X_l, \qquad \text{where} \qquad X_l=\sum\limits_{j=1}^{m_l} \one_{\{l\overset{j}{\rightsquigarrow}v\}}}~.
	}
	{By} Theorem~\ref{thm:equiv:PU:PAri}, model (D) is equal in distribution to P\'olya urn graph. % Let $\mathcal{E}$ be an event such that the bound on the attachment probabilities in Lemma~\ref{lem:bound:attachment_probability} holds true. Now from Lemma~\ref{lem:bound:attachment_probability}, we can say that $\prob\left(\mathcal{E}\right)>1-\varepsilon$. 
	Therefore,
	\eqan{\label{for:claim:bad:events:2}
		\E_{m}\left[d_v(n)^2\one_\mathcal{E}\right] =& \E_{m}\Big[ \Big( m_v+\sum\limits_{l=v+1}^n X_l \Big)^2\one_\mathcal{E} \Big]\nn\\
		\leq&  2m_v^2 + 2\E_{m}\Bigg[\Big( \sum\limits_{l=v+1}^n X_l \Big)^2\one_{\mathcal{E}_{\sss \hat{\chi},\psi}}\one_{\mathcal{E}_m}\Bigg]\nn\\
		=&2m_v^2 + 2\E_{m}\Bigg[\E_{m,\psi}\Big( \sum\limits_{l=v+1}^n X_l \Big)^2\one_{\mathcal{E}_{\sss \hat{\chi},\psi}}\Bigg]\one_{\mathcal{E}_m}~.}
	Now conditionally on $\boldsymbol{m,\psi},~(X_l)_{l\in(v,n]}$ are independent $\mathrm{Binom}(m_l,p_l)$ random variables, where $p_l=\prob_{m,\psi}(l\rightsquigarrow v)$. Using this independence in the second term of the RHS of \eqref{for:claim:bad:events:2}, we obtain
	\eqn{\label{for:claim:bad:event:2}
		\begin{split}
			\E_{m,\psi}\Big[ \sum\limits_{l=v+1}^n X_l \Big]^2 &= \sum\limits_{l=v+1}^n {\var}_{m,\psi} (X_l)+\Big( \sum\limits_{l=v+1}^n \E_{m,\psi}[X_l] \Big)^2\\
			&= \sum\limits_{l=v+1}^n m_lp_l(1-p_l) + \Big( \sum\limits_{l=v+1}^n m_lp_l \Big)^2.
	\end{split}}
	Following the same line of proof as in Lemma~\ref{lem:NFE:main} and using properties of $\mathcal{E}_{\sss \hat{\chi},\psi}$, we can show that conditionally on $\boldsymbol{m},\boldsymbol{\psi}$,
	\eqan{\label{for:claim:bad:events:3}
		\Big(\sum\limits_{l=v+1}^n m_l p_l(1-p_l)\Big)\one_{\mathcal{E}_{\sss \hat{\chi},\psi}}&\leq \Big(\sum\limits_{l=v+1}^n m_l p_l\Big)\one_{\mathcal{E}_{\sss \hat{\chi},\psi}} \nn\\
		&\hspace{0.25cm}\leq  2\hat{\chi}_v (\eta^\prime)^{\chi-1}\Big(\frac{1}{n}\sum\limits_{u\geq \eta^\prime n}m_u\left( \frac{u}{n} \right)^{-\chi}\Big)
		~.}
	Therefore, using property~\eqref{reg:4} of $\mathcal{E}_m$ and substituting the bound of \eqref{for:claim:bad:events:3} in \eqref{for:claim:bad:event:2},
	\eqan{\label{for:claim:bad:events:4}
		%&\E_{m,\mathcal{E}} \Big[\sum\limits_{l=v+1}^n m_l p_l\Big] \leq k_1 \E_{m,\mathcal{E}} [\hat{\chi}_v]\leq c_1 m_v~,\\
		\E_{m} \Big[\Big(\sum\limits_{l=v+1}^n m_l p_l\Big)^2\one_{\mathcal{E}_{\sss \hat{\chi},\psi}}\Big]\one_{\mathcal{E}_{m}} \leq 4c_0^2 \E_{m} [\hat{\chi}_v^2]\leq c_2 m_v^2~,}
	for some $c_2>0$. Choosing $c_1=2(1+c_0+c_2^2)$, for $v\geq \eta^\prime n,$ \eqref{lem:eq:degree_bound} holds true.
\end{proof}
\paragraph{\bf Proof of Lemma~\ref{lem:conditional:control:bad_events}} 
%To prove Lemma~\ref{lem:conditional:control:bad_events} we bound the LHS {of \eqref{lem:eq:conditional:control:bad_events}} by the total variation distance between $D_1^{\sss(n)}$ and $D_2^{\sss(n)}$. 
To prove Lemma~\ref{lem:conditional:control:bad_events}, we construct the following:
\eqan{\label{new:proof:1}
	{\rm{GOOD}}_n=&\{u:d_u^{\sss(D)}(n-1)=d_u^{\sss(E)}(n-1)\},\\
	{\rm{BAD}}_n=&\{u:d_u^{\sss(D)}(n-1)\neq d_u^{\sss(E)}(n-1)\},\nn
}
where \(d_u^{\sss(D)}(n-1)\) and \(d_u^{\sss(E)}(n-1)\), denotes the degree of vertex \(u\) in the coupled graphs \(\hat{G}_n\) and \(\hat{G}_n^\prime\).
Note that, the conditional event in the LHS of \eqref{lem:eq:conditional:control:bad_events} implies that \(v\in{\rm{GOOD}}_n\). Let, \(\tau_v\) denotes the first edge from \(n\) that connects to \(v\) in \(\hat{G}_n\). Then, from the optimal coupling \(\{D^{\sss(n,j)}:j\in[m_n]\}\), for any \(j>\tau_v,~\one_{\{{\bf{e}}_n^{i}=v\}}\) stochastically dominates \(\one_{\{{\bf{f}}_n^{i}=v\}}\). Therefore, unless
%Further, from the optimal coupling \(\{D^{\sss(n,j)}:j\in[m_n]\},~\one_{{\bf{f}}_n^{i}}\) stochastically dominates if vertex \(n\) connects to \(v\) with the first edge in model (D), then it connects to \(v\) with its first edge in model (E) as well, and vice versa. Subsequent connections to \(v\) from \(n\) in model (E) leads to the same connection in model (D), but not the other way round, leading to the event \(A_n\). On the other hand, if \(n\) doesn't connect to \(v\) with its first edge in \(\hat{G}_n\), it doesn't connect in \(\hat{G}_n^\prime\) as well. In this scenario, Subsequent connections to \(v\) from \(n\) in model (D) leads to the same connection in model (E), but not the other way round. 




Define,
\eqn{
	\label{new:proof:2}
	\mathbb{C}_1=\sum\limits_{i\in[m_n]}\one_{\{{\bf{e}}_n^{i}=v\}},\quad\text{and}\quad \mathbb{C}_2=\sum\limits_{i\in[m_n]}\one_{\{{\bf{f}}_n^{i}=v\}}~.
}
Therefore, from the optimal coupling \(\{D^{\sss(n,j)}:j\in[m_n]\}\), conditionally on \(\bigcap\limits_{h=v+1}^{n-1}A_h^c\bigcap\mathcal{E},~\mathcal{C}_1\succeq\mathcal{C}_2\) when \({\bf{e}}_n^1=v\) and \(\mathcal{C}_2\)  \(\mathcal{C}_1\) when \({\bf{e}}_n^1\neq v\)


In $\PArf_n(\boldsymbol{m},\delta)$, 
conditionally on $\boldsymbol{m}$ and $d_{v}(n-1)=d$, the probability of having $k$ connections from $n$ to $v$ and $m_n-k$ connections to other vertices in $[n-1]$ is given by
\eqn{\label{for:lem:bad:events:2}
	Q_k = \binom{m_n}{k}(p^\prime)^k(1-p^\prime)^{m_n-k},}
where $p^\prime= {(d+\delta)/(a_{[2]}+2\left( m_{[n-1]}-2 \right)+(n-1)\delta)}$ {is} as defined in \eqref{edge:probability:F}. On the other hand, in $\PAri_n(\boldsymbol{m},\delta)$, conditionally on $\boldsymbol{m}$ and $d_v(n-1)=d$, the {probability of the same event} is
\eqn{
	\label{for:lem:bad:events:3}
	T_k=\binom{m_n}{k}\prod\limits_{l=0}^{k-1}p_l(k)\prod\limits_{l=k}^{m_n-1}(1-p_l(k)),
}
where 
\[
p_l(k)=\begin{cases}
	&\frac{d+l+\delta}{a_{[2]}+2\left( m_{[n-1]}-2 \right)+l+(n-1)\delta},\quad\text{for}~l<k,\\
	&\frac{d+k+\delta}{a_{[2]}+2\left( m_{[n-1]}-2 \right)+l+(n-1)\delta},\quad\text{for}~l\geq k.
\end{cases}
\]
The exchangeability {of} model (D) {implies} that the probability of connecting any $k$ edges from $n$ to $v$ is {the} same, {which explains \eqref{for:lem:bad:events:3}}. 













Then, {again} conditionally on $\boldsymbol{m},$ and $d_{v}(n-1)=d$, the total variation distance between $D_1^{\sss(n)}$ and $D_2^{\sss(n)}$ is given by
\eqan{\label{for:lem:bad:events:4}
	d_{\sss\rm{TV}}\left( D_1^{\sss(n)},D_2^{\sss(n)} \right) =& \frac{1}{2}\sum\limits_{k=0}^{m_n}\left| Q_k-T_k \right|\nn\\
	\leq& \frac{1}{2}\left[ |Q_0-T_0|+|Q_1-T_1|+\sum\limits_{k=2}^{m_n}Q_k+\sum\limits_{k=2}^{m_n}T_k \right].
}
For the first two terms we use the telescoping bound in {\cite[equation (27)]{BergerBorgs} that reads}
\eqn{\label{eq:bound:BergerBorgs}
	\left| Q_k-T_k \right|\leq \binom{m_n}{k}\left[ \Tilde{p}^{k-1}\sum\limits_{l=0}^{k-1}\left| p^\prime-p_l(k) \right| + (p^\prime)^k\sum\limits_{l=k}^{m_n}\left| p^\prime-p_l(k) \right|  \right],
}
where $\Tilde{p}=\max\{ p^\prime, p_0(k),\ldots,p_{m_n}(k) \}$. For $k=0$ and $1$, the above bound gives
\eqn{
	\label{for:lem:bad:events:5}
	|Q_0-T_0|+|Q_1-T_1| \leq c_0m_n^2(d+\delta+1)^2 n^{-2}.
}

For the last term in the RHS of \eqref{for:lem:bad:events:4}, we {use that $T_k$ equals} the probability that exactly $k$ out-edges from vertex $n$ {connect} to vertex $v$ in model (D). Conditionally on $\boldsymbol{m},$ let $\prob_{m}^{\sss\rm{(D)}}$ denote the law for model (D).
Next we {condition} on the event that the first $2$ out-edges from $n$ connect to $v$, which is denoted by $n\overset{1,2}{\rightsquigarrow}v$.
\eqan{\label{for:lem:bad:events:7}
	%\begin{split}
	\sum\limits_{k=2}^{m_n}T_k=&\sum\limits_{k=2}^{m_n}\binom{m_n}{k}\prob_{m}^{\sss\rm{(D)}}\left( n\rightsquigarrow v\ \text{with its first $k$ edges} \right)\nn\\
	\leq&~ \frac{m_n^2}{2}\prob_{m}^{\sss\rm{(D)}}\left( n\overset{1,2}{\rightsquigarrow} v\right)\sum\limits_{k=2}^{m_n}\binom{m_n-2}{k-2}\prob_{m}^{\sss\rm{(D)}}\left( n\rightsquigarrow v\ \text{with first $k$ edges}\left| n\overset{1,2}{\rightsquigarrow} v\right. \right)\nn\\
	\leq&~ \frac{m_n^2(d+\delta+1)^2}{2n^2}.
	%\end{split}
}
The last inequality is obtained by substituting the first and second edge-connection probabilities from $n$ to $v$ and the conditional probabilities {sum} to $1$.
Similarly for model (E), if $\prob_{m}^{\sss\rm{(E)}}$ denotes the conditional law for model (E), then the probability of connecting more than $1$ edge from $n$ to $v$ can be bounded as \eqan{\label{for:lem:bad:events:8}
	%\begin{split}
	\sum\limits_{k=2}^{m_n}Q_k=&\sum\limits_{k=2}^{m_n}\binom{m_n}{k}\prob_{m}^{\sss\rm{(E)}}\left( n\rightsquigarrow v\ \text{with its first $k$ edges} \right)\nn\\
	\leq&~ \frac{m_n^2}{2}\prob_{m,}^{\sss\rm{(E)}}\left( n\overset{1,2}{\rightsquigarrow} v\right)\sum\limits_{k=2}^{m_n}\binom{m_n-2}{k-2}\prob_{m}^{\sss\rm{(E)}}\left( n\rightsquigarrow v\ \text{with first $k$ edges}\left| n\overset{1,2}{\rightsquigarrow} v\right. \right)\nn\\
	\leq&~ \frac{m_n^2(d+1)^2}{2n^2}.
	%\end{split}
}
On the other hand, the total variation distance {is} bounded by $1$. Therefore, collecting the bounds for all the contributions, conditionally on $\boldsymbol{m},$ we obtain
\eqn{
	\label{for:lem:bad:events:9}
	d_{\sss\rm{TV}}\left( D_1^{\sss(n)},D_2^{\sss(n)} \right) \leq 1\wedge \frac{c_0m_n^2 (d_{v}(n-1)+\delta+\delta)^2}{n^2}~,
}
%By \eqref{for:lem:bad:events:9} and Lemma~\ref{Lem:auxiliary:control:bad_event}, conditionally on $\boldsymbol{m}$ and $\mathcal{E},$
%\eqn{\label{for:lem:bad:events:10}
	%d_{\sss\rm{TV}}\left( D_1^{\sss(n)},D_2^{\sss(n)} \right) \leq 1\wedge \frac{c_0 m_n^2 m_v^2}{n^2}~.
	%}
for some constant $c_0>0$. Therefore, 
\eqan{\label{for:lem:bad:events:11}
	%\begin{split}
	\prob\left( A_n\cap\mathcal{E}\left|\bigcap\limits_{h=v+1}^{n-1} A_h^c\cap \mathcal{E}\right. \right) \leq& \E\left[ d_{\sss\rm{TV}}\left( D_1^{\sss(n)},D_2^{\sss(n)} \right)\one_\mathcal{E} \right]\nn\\
	\leq& \E\left[ 1\wedge \frac{c_0 m_n^2 \E_m[d_{v}(n-1)^2\one_\mathcal{E}]}{n^2} \right]~.
	%\end{split}
}
By Lemma~\ref{Lem:auxiliary:control:bad_event}, we can bound the conditional probability on the LHS of \eqref{for:lem:bad:events:11} by
\eqan{\label{for:lem:bad:events:11-1}
	%\begin{split}
	&\E\left[ 1\wedge \frac{c_0 c_1^2 m_n^2 m_v^2}{n^2} \right]\nn\\
	=&\prob\Big( m_nm_v>\frac{n}{c_1\sqrt{c_0}} \Big)+\frac{c_0c_1^2}{n^2}\E\left[ m_n^2m_v^2\one_{\{m_vm_n\leq \frac{n}{c_1\sqrt{c_0}}\}} \right]~,
	%\end{split}
}
where $c_0$ is as defined in Lemma~\ref{Lem:auxiliary:control:bad_event}. Since $(m_v)_{v\geq 3}$ have finite $(1+p)$-th moment, by Markov's inequality,
\[
\prob(m_v>x)\leq c_2x^{-(1+p)}.
\]
Using the independence of $m_n$ and $m_v$ and the above inequality, we can bound the first probability in \eqref{for:lem:bad:events:11-1} by Markov's inequality as
\eqn{\label{for:lem:bad:events:12}
	\prob\left( m_nm_v>\frac{n}{c_1\sqrt{c}} \right) \leq c_3\E\big[(m_nm_v)^{1+p}\big] n^{-(1+p)}= o(n^{-1})~.
}
%\RvdH{This is not obvious. Note that if $\prob(m_v>x)\leq c_1x^{-(1+p)},$ then $\prob(m_vm_n>x)\leq c_1x^{-(1+p)}\log{x}$. Explain in more detail.}
%\RR{Done!}
The {second term in \eqref{for:lem:bad:events:11-1} can} be written explicitly as
\eqan{
	\label{for:lemP:bad:events:13}
	\E\left[ m_n^2m_v^2\one_{\{m_vm_n\leq x \}} \right]
	\leq& c_3\sum\limits_{k=1}^x k \prob(m_nm_v>k)\nn\\
	\leq& c_4\E\big[(m_nm_v)^{1+p}\big]\sum\limits_{k=1}^x k^{-p}\leq c_5 x^{1-p}~.
}
for some positive finite constants $c_3,~c_4$ and $c_5$. Substituting the bounds obtained from \eqref{for:lem:bad:events:12} and \eqref{for:lemP:bad:events:13} in \eqref{for:lem:bad:events:11} yields,
\[
\prob\left( A_n\cap\mathcal{E}\left|\bigcap\limits_{h=v+1}^{n-1} A_h^c\cap \mathcal{E}\right. \right) \leq c_5 n^{-(1+p)}=o\left( n^{-1} \right).
\]
This completes the proof of Lemma~\ref{lem:conditional:control:bad_events}.
{\qed}
%\smallskip

The only difference between model (E) and (F) is that model (F) does {not} allow for multiple connections between two vertices, {while model (E) does. Thus,} model (F) and (D) could be coupled in a similar way with some minor adaptations:

\begin{Proposition}[Coupling between models (D) and (F)]{\label{prop:coupling:D:F}}
	{The statement in Proposition \ref{prop:coupling:D:E} also holds for models (D) and (F).}
\end{Proposition}
\begin{remark}[Local convergence for model (F)]
	\rm\chRounak{Similar to model (E), the proof for the local convergence of model (F) to the random P\'{o}lya point tree follows immediately subject to Proposition~\ref{prop:coupling:D:F}.}
\end{remark}
The proof to Proposition~\ref{prop:coupling:D:F} follows exactly the same argument as {that of} Proposition~\ref{prop:coupling:D:E}. To prove Proposition~\ref{prop:coupling:D:E}, we needed Lemma~\ref{lem:conditional:control:bad_events} and \ref{Lem:auxiliary:control:bad_event}. Lemma~\ref{Lem:auxiliary:control:bad_event} proves a property {of} model (D), {and thus we do not} need to adapt this lemma. Additionally, subject to Lemma~\ref{lem:conditional:control:bad_events}, the proof {of} Proposition~\ref{prop:coupling:D:E} does not use any property of model (E). {Thus,} if we manage to {adapt Lemma~\ref{lem:conditional:control:bad_events} to} model (F), {the} proof {of} Proposition~\ref{prop:coupling:D:F} follows immediately. 

For the proof {of Lemma~\ref{lem:conditional:control:bad_events} for model (F),} we construct a similar coupling between model (D) and (F) as we {have} constructed for model (D) and (E) earlier in this Section. Then we claim that Lemma~\ref{lem:conditional:control:bad_events} also holds {for} model (F).



\begin{proof}[\bf Proof of Lemma~\ref{lem:conditional:control:bad_events} for model (F)]
	Note that for model (F), there cannot be more than one edge between two vertices. Let $p_l^\prime$ denote the conditional edge-connection probability of connecting the $n$-th vertex to vertex $v$ with its $l$-th edge and $Q_k^\prime$ denote the probability of connecting $k$ edges from $n$ to $v$ in model (F). Then the total variation distance in \eqref{for:lem:bad:events:4} can be rewritten for model (F) as
	\eqan{\label{for:lem:model:F:1}
		d_{\sss\rm{TV}}\left( D_1^{\sss(n)}, D_2^{\sss(n)} \right)=&\frac{1}{2}\sum\limits_{k=0}^{m_n} \left| Q_k^\prime-T_k \right| \nn\\
		=& \frac{1}{2}\Big[ |Q_0^\prime-T_0|+|Q_1^\prime-T_1| +\sum\limits_{k=2}^{m_n} T_k \Big]~.}
	%\RvdH{Note that one of these terms can be omitted when we also remove the factor 1/2. This may be useful.}
	Since $\sum\limits_{k=0}^1 Q_k^\prime =\sum\limits_{k=0}^{m_n} T_k =1,$ we bound $|Q_1^\prime-T_1|$ as
	\eqn{\label{for:lem:model:F:1-1}\begin{split}
			|Q_1^\prime-T_1| = \big| (1-Q_0^\prime)-(1-T_0-\sum\limits_{k=2}^{m_n}T_k) \big| \leq |Q_0^\prime-T_0| + \sum\limits_{k=2}^{m_n}T_k~,
	\end{split}}
	and the total variation distance can be bounded by
	\eqn{\label{for:lem:model:F:1-2}
		d_{\sss\rm{TV}}\left( D_1^{\sss(n)}, D_2^{\sss(n)} \right)\leq |Q_0^\prime-T_0| + \sum\limits_{k=2}^{m_n}T_k}
	Therefore we do not need to bound $|Q_1^\prime-T_1|,$ if we manage to bound the RHS of \eqref{for:lem:model:F:1-2}.
	From \eqref{for:lem:bad:events:7}, we already have the required bound for $\sum\limits_{k=2}^{m_n} T_k$. For the other term in the RHS of \eqref{for:lem:model:F:1-2}, we use a triangle inequality argument {to} obtain
	\eqn{\label{for:lem:model:F:2}
		|Q_0^\prime-T_0|\leq |Q_0-T_0| + |Q_0^\prime-Q_0|~,}
	where $Q_k$ {is} defined in \eqref{for:lem:bad:events:2}. Therefore, again from \eqref{for:lem:bad:events:5}, we have the desired bound for the first term in the RHS of \eqref{for:lem:model:F:2}. Now we are left to show that the other term also has the same upper bound. Note that $p^\prime\leq p_l^\prime$ for all $l\geq 1$ and
	\eqn{\label{for:lem:model:F:2-1}
		p_{m_n}^\prime \leq \frac{d+\delta}{\sum\limits_{n\not\sim u}(d_{v}(n-1) + \delta)}~,}
	where $n\not\sim u$ implies that $u$ and $n$ are not connected by an edge.
	Let $\zeta_0=\delta+\infsupp(M)>0$. Then for all $u\in[n-1],~d_{v}(n-1)+\delta\geq \zeta_0$ and the denominator of the RHS of \eqref{for:lem:model:F:2-1} can be further lower bounded by $(n-m_n)\zeta_0$. On the event space $\mathcal{E},~m_n\leq n^{1-\varrho/2}.$ Therefore there exists another constant $\zeta_1>0,$ such that on $\mathcal{E},$ the denominator can be further lower bounded by $n\zeta_1$ and the LHS of \eqref{for:lem:model:F:2-1} can be upper bounded by $(d+\delta)/(n\zeta_1).$
	
	Therefore using the telescoping sum bound in \eqref{eq:bound:BergerBorgs}, we have upper bound for $|Q_0^\prime-Q_0|$. 
	%\RvdH{This is too fast, and note that we may choose not to bound $|Q_1-Q_1^\prime|$.}
	%\RR{Yes. we can stop here and remove the bound for $|Q_1-Q_1^\prime|$.}
\end{proof}

==> Chap5_Continuity_percolation/Chap5figs/CL.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[width = 0.98\linewidth,
 height=0.4\textwidth,
 axis lines=middle,
tick align=outside,
ticks=none,
 xlabel=$t$, % Label for x-axis
ylabel=$y$, % Label for y-axis
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-5.00554078958081, xmax=105.116356581197,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.533108429506719, ymax=11.1952770196411,
ytick style={color=black}
]
\addplot [semithick, Neongreen]
table {%
0 1
1.06376179464851 1.95738561518366
1.06376179464851 0.957385615183656
1.78793165395663 1.60913848856097
1.78793165395663 0.60913848856097
2.71194619421565 1.44075157479408
2.71194619421565 0.440751574794081
2.98171049828441 0.683539448455972
2.98171049828441 0
4.49515711784552 1.36210195760499
4.49515711784552 0.362101957604994
5.54436681499481 1.30639068503936
5.54436681499481 0.306390685039358
7.15615787749874 1.7570026412929
7.15615787749874 0.757002641292899
7.82346306054401 1.35757730603364
7.82346306054401 0.357577306033639
8.53525169556668 0.998187077554045
8.53525169556668 0
10.5348105575694 1.7996029758024
10.5348105575694 0.799602975802401
10.8047443434867 1.04254338312803
10.8047443434867 0.0425433831280264
10.8062975031513 0.0439412268261484
10.8062975031513 0
12.114842544676 1.17769053737222
12.114842544676 0.17769053737222
13.3868425550004 1.32249054666416
13.3868425550004 0.32249054666416
13.813460121674 0.70644635667043
13.813460121674 0
16.5294966791209 2.44443290170218
16.5294966791209 1.44443290170218
17.8387689557022 2.62277795062541
17.8387689557022 1.62277795062541
18.5738942808615 2.28439074326879
18.5738942808615 1.28439074326879
20.2149217342926 2.76131545135678
20.2149217342926 1.76131545135678
21.0836609544059 2.54318074945873
21.0836609544059 1.54318074945873
21.1949190680653 1.64331305175218
21.1949190680653 0.643313051752178
21.3739509103309 0.804441709791232
21.3739509103309 0
23.4265704429392 1.84735757934742
23.4265704429392 0.847357579347419
23.4971927209613 0.910917629567364
23.4971927209613 0
24.664319998526 1.05041454980821
24.664319998526 0.0504145498082145
28.255139355847 3.28215197139709
28.255139355847 2.28215197139709
28.4251420272481 2.43515437565814
28.4251420272481 1.43515437565814
29.2779329650768 2.20266621970395
29.2779329650768 1.20266621970395
30.5569032426015 2.35373946947621
30.5569032426015 1.35373946947621
30.839703170292 1.60825940439763
30.839703170292 0.608259404397628
30.9666234654398 0.722487670030679
30.9666234654398 0
31.1227001401308 0.140469007221822
31.1227001401308 0
31.1653856468875 0.0384169560810976
31.1653856468875 0
31.2124147324374 0.0423261769949148
31.2124147324374 0
31.3048404550312 0.0831831503343701
31.3048404550312 0
32.7248627974025 1.27802010813415
32.7248627974025 0.278020108134152
33.566603826869 1.03558703465405
33.566603826869 0.0355870346540524
34.9059450923159 1.24099417355627
34.9059450923159 0.240994173556269
35.9243441310685 1.15755330843361
35.9243441310685 0.157553308433607
36.8589717903666 0.998718201801893
36.8589717903666 0
39.322761581685 2.21741081218654
39.322761581685 1.21741081218654
42.7436332956732 4.29619535477595
42.7436332956732 3.29619535477595
45.2536516353076 5.55521186044689
45.2536516353076 4.55521186044689
46.1831202218363 5.39173358832272
46.1831202218363 4.39173358832272
47.7267644913108 5.7810134308498
47.7267644913108 4.7810134308498
49.9781948212244 6.80730072777205
49.9781948212244 5.80730072777205
50.3105158717775 6.10638967326976
50.3105158717775 5.10638967326976
52.6484102676486 7.21049462955379
52.6484102676486 6.21049462955379
53.3571914232827 6.84839766962451
53.3571914232827 5.84839766962451
54.6789117724701 7.03794598389317
54.6789117724701 6.03794598389317
58.5102889348863 9.48618543006773
58.5102889348863 8.48618543006773
60.175790580783 9.98513691137478
60.175790580783 8.98513691137478
62.0391591127381 10.6621685901344
62.0391591127381 9.66216859013437
62.6073683556599 10.1735569087639
62.6073683556599 9.17355690876394
62.9196429367169 9.45460403171529
62.9196429367169 8.45460403171529
63.0111214265834 8.53693467259511
63.0111214265834 7.53693467259511
63.9432917609802 8.37588797355223
63.9432917609802 7.37588797355223
64.0350823565308 7.4584995095478
64.0350823565308 6.4584995095478
64.2565493970876 6.6578198460489
64.2565493970876 5.6578198460489
66.6311379413731 7.79494953590586
66.6311379413731 6.79494953590586
66.8004406513788 6.94732197491094
66.8004406513788 5.94732197491094
67.347740923682 6.43989221998383
67.347740923682 5.43989221998383
67.4665895557559 5.54685598885034
67.4665895557559 4.54685598885034
67.7533162964741 4.80491005549676
67.7533162964741 3.80491005549676
68.6474972311957 4.60967289674622
68.6474972311957 3.60967289674622
68.7455621552653 3.69793132840887
68.7455621552653 2.69793132840887
69.6279369579094 3.49206865078854
69.6279369579094 2.49206865078854
70.0270942532766 2.85131021661897
70.0270942532766 1.85131021661897
70.6497079692049 2.41166256095449
70.6497079692049 1.41166256095449
71.5121000088835 2.18781539666521
71.5121000088835 1.18781539666521
71.6535762992363 1.31514405798272
71.6535762992363 0.315144057982716
77.983205369935 6.01181022161152
77.983205369935 5.01181022161152
78.8208520773616 5.76569225829545
78.8208520773616 4.76569225829545
78.9616481593737 4.89240873210637
78.9616481593737 3.89240873210637
81.9859578494346 6.61428745316114
81.9859578494346 5.61428745316114
83.0742176947783 6.59372131397054
83.0742176947783 5.59372131397054
83.2018610417735 5.70860032626622
83.2018610417735 4.70860032626622
84.0550230809263 5.47644616150374
84.0550230809263 4.47644616150374
85.2604676578113 5.56134628070024
85.2604676578113 4.56134628070024
86.1950471882218 5.40246785806967
86.1950471882218 4.40246785806967
87.8373131022991 5.88050718073923
87.8373131022991 4.88050718073923
87.9209851698212 4.95581204150914
87.9209851698212 3.95581204150914
88.0056019133447 4.0319671106803
88.0056019133447 3.0319671106803
88.0831295289014 3.10174196468129
88.0831295289014 2.10174196468129
88.6946760973437 2.65213387627941
88.6946760973437 1.65213387627941
93.8889561341353 6.32698590939179
93.8889561341353 5.32698590939179
94.3156671695722 5.71102584128504
94.3156671695722 4.71102584128504
95.6437649715555 5.90631386307001
95.6437649715555 4.90631386307001
96.3008789540648 5.49771644732842
96.3008789540648 4.49771644732842
96.8249115726064 4.96934580401582
96.8249115726064 3.96934580401582
97.4006493398584 4.48750979454264
97.4006493398584 3.48750979454264
97.4369186723913 3.52015219382228
97.4369186723913 2.52015219382228
97.5726622344669 2.64232139969031
97.5726622344669 1.64232139969031
98.9966485165536 2.9239090535683
98.9966485165536 1.9239090535683
99.369051610358 2.25907183799225
99.369051610358 1.25907183799225
99.982080046087 1.81079743014843
99.982080046087 0.810797430148427
100.110815791616 0.926659601124612
100.110815791616 0
};
\end{axis}

\end{tikzpicture}


==> Chap5_Continuity_percolation/Chap5figs/renewal_proc.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da7191067947252416] 
\draw    (100.27,31.1) -- (100.93,225.1) ;
%Straight Lines [id:da13200798777620082] 
\draw    (78.93,211.1) -- (412.24,210.14) ;
%Shape: Arc [id:dp8601596858651692] 
\draw  [draw opacity=0] (101.6,210.53) .. controls (106.37,197.87) and (122.21,188.51) .. (141.06,188.4) .. controls (160.33,188.29) and (176.56,197.88) .. (181.08,210.91) -- (141.24,218.4) -- cycle ; \draw   (101.6,210.53) .. controls (106.37,197.87) and (122.21,188.51) .. (141.06,188.4) .. controls (160.33,188.29) and (176.56,197.88) .. (181.08,210.91) ;  
%Shape: Arc [id:dp8290869440958257] 
\draw  [draw opacity=0] (181.08,210.91) .. controls (183.26,198.07) and (193.66,188.3) .. (206.22,188.23) .. controls (218.76,188.16) and (229.26,197.78) .. (231.6,210.57) -- (206.38,215.93) -- cycle ; \draw   (181.08,210.91) .. controls (183.26,198.07) and (193.66,188.3) .. (206.22,188.23) .. controls (218.76,188.16) and (229.26,197.78) .. (231.6,210.57) ;  
%Shape: Arc [id:dp4677217806206091] 
\draw  [draw opacity=0] (276.16,210.7) .. controls (277.74,199.31) and (286.08,190.6) .. (296.17,190.55) .. controls (306.32,190.49) and (314.79,199.18) .. (316.45,210.64) -- (296.31,214.7) -- cycle ; \draw   (276.16,210.7) .. controls (277.74,199.31) and (286.08,190.6) .. (296.17,190.55) .. controls (306.32,190.49) and (314.79,199.18) .. (316.45,210.64) ;  
%Shape: Arc [id:dp37216681968971166] 
\draw  [draw opacity=0] (316.45,210.64) .. controls (321.21,198.7) and (336.64,189.9) .. (354.99,189.8) .. controls (373.5,189.69) and (389.14,198.47) .. (393.89,210.51) -- (355.15,218.33) -- cycle ; \draw   (316.45,210.64) .. controls (321.21,198.7) and (336.64,189.9) .. (354.99,189.8) .. controls (373.5,189.69) and (389.14,198.47) .. (393.89,210.51) ;  
%Straight Lines [id:da18041443023784964] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (358.32,153.74) -- (358.32,209.74) ;
%Straight Lines [id:da1348644735044755] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (316.72,107.1) -- (316.45,210.64) ;
%Shape: Arc [id:dp8307295702583359] 
\draw  [draw opacity=0] (316.27,155.32) .. controls (318.57,144.85) and (327.25,137.08) .. (337.58,137.12) .. controls (347.33,137.15) and (355.56,144.13) .. (358.32,153.74) -- (337.49,160.85) -- cycle ; \draw   (316.27,155.32) .. controls (318.57,144.85) and (327.25,137.08) .. (337.58,137.12) .. controls (347.33,137.15) and (355.56,144.13) .. (358.32,153.74) ;  
%Shape: Arc [id:dp00922699109223668] 
\draw  [draw opacity=0] (100.09,102.27) .. controls (106.69,90.56) and (152.54,81.63) .. (208.09,81.83) .. controls (268.13,82.05) and (316.77,92.86) .. (316.72,105.97) .. controls (316.72,106.08) and (316.72,106.2) .. (316.71,106.31) -- (208,105.57) -- cycle ; \draw   (100.09,102.27) .. controls (106.69,90.56) and (152.54,81.63) .. (208.09,81.83) .. controls (268.13,82.05) and (316.77,92.86) .. (316.72,105.97) .. controls (316.72,106.08) and (316.72,106.2) .. (316.71,106.31) ;  
%Shape: Arc [id:dp04095482677186757] 
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (316.71,106.31) .. controls (318.03,93.79) and (338.41,83.9) .. (363.32,84) .. controls (388.12,84.09) and (408.36,94.03) .. (409.75,106.49) -- (363.24,107.73) -- cycle ; \draw  [dash pattern={on 0.84pt off 2.51pt}] (316.71,106.31) .. controls (318.03,93.79) and (338.41,83.9) .. (363.32,84) .. controls (388.12,84.09) and (408.36,94.03) .. (409.75,106.49) ;  
%Shape: Arc [id:dp9674879656102757] 
\draw  [draw opacity=0] (316.71,106.31) .. controls (318.03,93.79) and (338.41,83.9) .. (363.32,84) .. controls (377.49,84.05) and (390.18,87.32) .. (398.7,92.43) -- (363.24,107.73) -- cycle ; \draw   (316.71,106.31) .. controls (318.03,93.79) and (338.41,83.9) .. (363.32,84) .. controls (377.49,84.05) and (390.18,87.32) .. (398.7,92.43) ;  

% Text Node
\draw (128.32,218.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{1}$};
% Text Node
\draw (196.72,218.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{2}$};
% Text Node
\draw (277.92,219.78) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{B_{k}( x)}$};
% Text Node
\draw (332.32,219.78) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{B_{k}( x) +1}$};
% Text Node
\draw (357.92,195.58) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle x$};
% Text Node
\draw (323.52,112.14) node [anchor=north west][inner sep=0.75pt]    {$U_{k}( x)$};
% Text Node
\draw (160.72,28.74) node [anchor=north west][inner sep=0.75pt]   [align=left] {Transactions in $ $\\block $\displaystyle k$};
% Text Node
\draw (328.72,33.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {Transactions in\\ block $\displaystyle k+1$};
% Text Node
\draw (81.6,6.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle N_{k}( t)$};
% Text Node
\draw (416.27,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle t$};


\end{tikzpicture}

